Foundational Large Language Models for Materials Research

Materials discovery and development are critical for addressing global challenges. Yet, the exponential growth in materials science literature comprising vast amounts of textual data has created significant bottlenecks in knowledge extraction, synthesis, and scientific reasoning. Large Language Models (LLMs) offer unprecedented opportunities to accelerate materials research through automated analysis and prediction. Still, their effective deployment requires domain-specific adaptation for understanding and solving domain-relevant tasks. Here, we present LLaMat, a family of foundational models for materials science developed through continued pretraining of LLaMA models on an extensive corpus of materials literature and crystallographic data. Through systematic evaluation, we demonstrate that LLaMat excels in materials-specific NLP and structured information extraction while maintaining general linguistic capabilities. The specialized LLaMat-CIF variant demonstrates unprecedented capabilities in crystal structure generation, predicting stable crystals with high coverage across the periodic table. Intriguingly, despite LLaMA-3's superior performance in comparison to LLaMA-2, we observe that LLaMat-2 demonstrates unexpectedly enhanced domain-specific performance across diverse materials science tasks, including structured information extraction from text and tables, more particularly in crystal structure generation, a potential adaptation rigidity in overtrained LLMs. Altogether, the present work demonstrates the effectiveness of domain adaptation towards developing practically deployable LLM copilots for materials research. Beyond materials science, our findings reveal important considerations for domain adaptation of LLMs, such as model selection, training methodology, and domain-specific performance, which may influence the development of specialized scientific AI systems.

==> layout.tex <==

Methodology:
1. Dataset
    1. pretraining
    2. finetuning
    3. Downstream

2. Training methodology
    1. pretraining
    2. finetuning
    3. Downstream

3. Evaluation
    1. Metrics - p,r,f1, loss
    2. Downstream 
    3. IE tasks

4. Hardware details
    cerebras 
    nvidia a100

==> todo.tex <==
Methodology:
1. Dataset
    1. pretraining
    2. finetuning
    3. Downstream
    4. Nate gruver

2. Training methodology
    1. pretraining
    2. finetuning
    3. Downstream
    4. Energy calculations and CIF

3. Evaluation
    1. Metrics - p,r,f1, loss
    2. Downstream - 3 seeds check
    3. IE tasks
    4. Discomat and matbookqa - Z
    5. CIF evaluation - Z, VB
    
4. Hardware details
    cerebras - B
    nvidia a100 - D


Results and discussion

Introduction

Conclusion

Abstract

#########Vaibhav Bihani ##############
Models : CHGNet, M3GNet, MACE
llamat2 : chgnet, m3gnet, mace
llamat3 :   #   , m3gnet,  #


